The supernova impostor PSN J09132750+7627410 and its progenitor

We report the results of our follow-up campaign of the supernova impostor PSN J09132750+7627410, based on optical data covering $\sim250\,\rm{d}$. From the beginning, the transient shows prominent narrow Balmer lines with P-Cygni profiles, with a blue-shifted absorption component becoming more prominent with time. Along the $\sim3\,\rm{months}$ of the spectroscopic monitoring, broad components are never detected in the hydrogen lines, suggesting that these features are produced in slowly expanding material. The transient reaches an absolute magnitude $M_r=-13.60\pm0.19\,\rm{mag}$ at maximum, a typical luminosity for supernova impostors. Amateur astronomers provided $\sim4\,\rm{years}$ of archival observations of the host galaxy, NGC 2748. The detection of the quiescent progenitor star in archival images obtained with the Hubble Space Telescope suggests it to be an $18-20$\msun white-yellow supergiant.

==> MRT.tex <==

\begin{deluxetable}{ccccccccccccl}
\tablecaption{Historical $r$-band light-curve}
\tablehead{\colhead{Date} & \colhead{MJD} & \colhead{$W1$(err)} & \colhead{$M2$(err)} & \colhead{$W2$(err)} & \colhead{$u$(err)} & \colhead{$g$(err)} & \colhead{$r$(err)} & \colhead{$i$(err)} & \colhead{$z$(err)} & \colhead{$B$(err)} & \colhead{$V$(err)} & \colhead{Instrument} }
\startdata
20110206 & 55598.03 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.7$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20110225 & 55617.02 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.9$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20110323 & 55643.96 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20110402 & 55653.99 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.6$     & \nodata     & \nodata     & \nodata     & \nodata     & KAF0260	           \\
20110513 & 55694.94 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20110614 & 55726.96 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>17.7$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20110804 & 55777.93 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20110926 & 55830.00 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20111023 & 55857.95 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20111115 & 55880.86 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.8$     & \nodata     & \nodata     & \nodata     & \nodata     & TRICOLOR         \\
20111116 & 55881.98 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20111121 & 55886.82 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>20.3$     & \nodata     & \nodata     & \nodata     & \nodata     & TRICOLOR         \\
20111218 & 55913.17 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20120107 & 55933.03 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.6$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20120220 & 55977.72 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.4$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20120319 & 56005.86 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.6$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20120428 & 56045.11 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.7$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20120602 & 56080.95 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20120710 & 56118.98 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.5$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20121203 & 56264.91 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20121219 & 56280.98 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130203 & 56326.89 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130215 & 56338.97 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.9$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130312 & 56363.81 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130407 & 56389.96 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.4$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130603 & 56446.87 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130702 & 56475.95 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.1$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130901 & 56536.80 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130902 & 56537.79 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.1$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130902 & 56537.87 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.2$     & \nodata     & \nodata     & \nodata     & \nodata     & SDI	           \\
20130902 & 56537.96 & \nodata     & \nodata     & \nodata    & \nodata      & \nodata    &   $>20.2$    & $>20$      &  \nodata     & $>20.4$    & $>20$      & AFOSC \\
20130903 & 56538.79 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.5$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130904 & 56539.79 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.0$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130906 & 56541.78 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.4$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130912 & 56547.78 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20130920 & 56555.78 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140209 & 56697.80 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>19.0$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140308 & 56724.89 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.9$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140323 & 56739.86 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140413 & 56760.93 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.7$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140517 & 56794.97 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140605 & 56813.94 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.3$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140828 & 56897.80 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.8$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140914 & 56914.77 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20140929 & 56929.77 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.6$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20141223 & 57014.93 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.9$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20150106 & 57028.90 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>18.2$     & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20150202 & 57055.89 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & 18.61(0.43) & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20150212 & 57065.04 & \nodata     & \nodata     & \nodata     & 17.73(0.04) & 18.49(0.08) & 18.35(0.06) & 18.41(0.07) & 18.63(0.24) & 18.61(0.04) & 18.45(0.03) & AFOSC            \\
20150212 & 57065.81 & 18.30(0.47) & 18.76(0.31) & 19.13(0.19) & 17.61(0.21) & \nodata     & \nodata     & \nodata     & \nodata     & 18.55(0.13) & 18.44(0.34) & UVOT             \\
20150214 & 57067.06 & $>18.1$     & $>18.5$     & 18.87(0.07) & 17.51(0.15) & \nodata     & \nodata     & \nodata     & \nodata     & 18.56(0.17) & 18.29(0.28) & UVOT             \\
20150216 & 57069.50 & 18.24(0.17) & $>18.3$     & 19.03(0.12) & 17.68(0.16) & \nodata     & \nodata     & \nodata     & \nodata     & 18.51(0.20) & $>18.2$     & UVOT             \\
20150216 & 57069.76 & \nodata     & \nodata     & \nodata     & 17.66(0.07) & 18.34(0.08) & 18.34(0.06) & 18.27(0.05) & \nodata     & 18.53(0.03) & 18.27(0.03) & AFOSC            \\
20150218 & 57071.22 & 18.43(0.11) & 19.02(0.19) & $>19.21$    & 17.85(0.16) & \nodata     & \nodata     & \nodata     & \nodata     & 18.57(0.10) & 18.34(0.30) & UVOT             \\
20150218 & 57071.96 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & 18.29(0.36) & \nodata     & \nodata     & \nodata     & \nodata     & Starlight SXVR H9 \\
20150220 & 57073.12 & \nodata     & \nodata     & \nodata     & 17.94(0.06) & 18.41(0.04) & 18.37(0.09) & 18.17(0.14) & \nodata     & 18.47(0.06) & 18.31(0.03) & AFOSC            \\
20150222 & 57075.31 & 18.62(0.13) & $>18.9$     & 19.39(0.18) & 18.13(0.18) & \nodata     & \nodata     & \nodata     & \nodata     & 18.52(0.34) & 18.36(0.18) & UVOT             \\
20150310 & 57091.02 & \nodata     & \nodata     & \nodata     & \nodata     & 18.91(0.08) & 18.65(0.08) & 18.22(0.06) & \nodata     & \nodata     & 18.66(0.20) & AFOSC            \\
20150311 & 57092.51 & 18.82(0.42) & 19.36(0.26) & $>19.7$     & 19.15(0.41) & \nodata     & \nodata     & \nodata     & \nodata     & 18.91(0.23) & $>18.2$     & UVOT             \\
20150311 & 57092.88 & \nodata     & \nodata     & \nodata     & \nodata     & 18.72(0.04) & 18.51(0.03) & 18.16(0.08) & \nodata     & 19.04(0.05) & 18.62(0.03) & AFOSC            \\
20150319 & 57100.01 & \nodata     & \nodata     & \nodata     & \nodata     & 18.92(0.05) & 18.59(0.06) & 18.19(0.06) & \nodata     & 19.19(0.08) & 18.73(0.04) & AFOSC            \\
20150326 & 57107.90 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & 18.68(0.14) & \nodata     & \nodata     & \nodata     & \nodata     & OSIRIS           \\
20150327 & 57108.87 & \nodata     & \nodata     & \nodata     & \nodata     & $>19.0$     & 18.77(0.08) & 18.49(0.09) & \nodata     & $>19.2$     & 19.18(0.18) & AFOSC            \\
20150330 & 57111.82 & \nodata     & \nodata     & \nodata     & \nodata     & $>19.2$     & 18.88(0.04) & 18.52(0.08) & $>18.5$     & $>19.2$     & 19.32(0.18) & AFOSC            \\
20150413 & 57125.82 & \nodata     & \nodata     & \nodata     & \nodata     & $>19.1$     & 19.33(0.12) & 18.75(0.12) & \nodata     & \nodata     & $>17.8$     & AFOSC            \\
20150415 & 57125.82 & \nodata     & \nodata     & \nodata     & 21.55(0.28) & \nodata     & \nodata     & \nodata     & 18.90(0.05) & $>20.4$     & \nodata     & AFOSC            \\
20150428 & 57140.88 & \nodata     & \nodata     & \nodata     & \nodata     & 20.96(0.08) & 19.51(0.08) & 18.70(0.08) & 18.86(0.10) & \nodata     & \nodata     & ALFOSC\_FASU     \\
20150508 & 57150.97 & \nodata     & \nodata     & \nodata     & \nodata     & 21.10(0.04) & 19.58(0.07) & 19.00(0.06) & 18.96(0.14) & \nodata     & \nodata     & ALFOSC\_FASU     \\
20150518 & 57160.92 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & 19.64(0.06) & \nodata     & \nodata     & \nodata     & \nodata     & OSIRIS           \\
20150525 & 57167.96 & \nodata     & \nodata     & \nodata     & \nodata     & 21.62(0.09) & 19.92(0.08) & 19.01(0.14) & 18.97(0.16) & 22.41(0.09) & 20.64(0.09) & ALFOSC\_FASU     \\
20150610 & 57183.89 & \nodata     & \nodata     & \nodata     & \nodata     & $>20.9$     & 20.23(0.12) & 19.38(0.06) & 19.29(0.19) & \nodata     & 20.75(0.20) & AFOSC            \\
20150622 & 57195.92 & \nodata     & \nodata     & \nodata     & $>21.3$     & 22.28(0.08) & 20.74(0.04) & 19.72(0.08) & 19.73(0.23) & $>22.8$     & 21.47(0.22) & ALFOSC\_FASU     \\
20150709 & 57212.91 & \nodata     & \nodata     & \nodata     & \nodata     & $>22.7$     & 21.78(0.12) & 20.50(0.07) & 20.58(0.12) & $>22.6$     & 22.28(0.18) & ALFOSC\_FASU     \\
20150714 & 57217.86 & \nodata     & \nodata     & \nodata     & \nodata     & $>22.2$     & $>21.7$     & 20.69(0.24) & \nodata     & \nodata     & \nodata     & AFOSC            \\
20150717 & 57220.96 & \nodata     & \nodata     & \nodata     & $>20.5$     & $>22.4$     & $>21.9$     & 20.86(0.26) & 21.05(0.39) & $>21.5$     & $>21.8$     & AFOSC            \\
20150723 & 57226.90 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>22.4$     & 21.42(0.39) & \nodata     & \nodata     & \nodata     & ALFOSC\_FASU     \\
20151106 & 57332.16 & \nodata     & \nodata     & \nodata     & \nodata     & $>22.9$     & $>21.7$     & $>21.4$     & \nodata     & $>22.8$     & $>22.6$     & AFOSC            \\
20151109 & 57335.12 & \nodata     & \nodata     & \nodata     & \nodata     & \nodata     & $>22.9$     & \nodata     & \nodata     & \nodata     & \nodata     & AFOSC            \\
\enddata
\tablecomments{Historical data (from 2011 February 6 to 2015 January 6), provided by Giancarlo Cortini, using a $0.35\,\rm{m}$ Schmidt-Cassegrain (C14) with a Starlight SXVR H9 camera equipped with a Sony ICX 285 sensor (Osservatorio Astronomico di Monte Maggiore - Predappio (FC)), by Fabio Martinelli, using a $0.35\,\rm{m}$ Schmidt-Cassegrain (C14) with a CCD camera KAF0260 and by Riccarco Mancini with a $0.25\,\rm{m}$ Newtonian telescope with a CCD camera Meade SDI Pro-d. These were unfiltered images and have been re-scaled to the $r$-band in the AB photometric system. Additional photometric limits were obtained on 2011 November 15 ($g>19.2$, $i>19.2$), 2011 November 21 ($g>19.5$, $i>19.7$) using the 0.105~m Schmidt Telescope located at the Kiso Observatory of the Institute of Astronomy of the University of Tokyo and the KWFC camera, and 2013 February 19 ($i>17.6$) using the GRB~0.5~m telescope located at the Okayama Astrophysical Observatory (National Astronomical Observatory of Japan) and the TRICOLOR camera.
Optical and UV observations (from 2015 February 12) were carried out using the instruments described in the paper.
}
\end{deluxetable}

